Tip of the Red Giant Branch Distances with JWST. II. I-band Measurements in a Sample of Hosts of 10 SN Ia Match HST Cepheids

The Hubble Tension, a >5 sigma discrepancy between direct and indirect measurements of the Hubble constant (H0), has persisted for a decade and motivated intense scrutiny of the paths used to infer H0. Comparing independently-derived distances for a set of galaxies with different standard candles, such as the tip of the red giant branch (TRGB) and Cepheid variables, can test for systematics in the middle rung of the distance ladder. The I band is the preferred filter for measuring the TRGB due to constancy with color, a result of low sensitivity to population differences in age and metallicity supported by stellar models. We use James Webb Space Telescope (JWST) observations with the maser host NGC 4258 as our geometric anchor to measure I-band (F090W vs F090W-F150W) TRGB distances to 8 hosts of 10 Type Ia supernovae (SNe Ia) within 28 Mpc: NGC 1448, NGC 1559, NGC 2525, NGC 3370, NGC 3447, NGC 5584, NGC 5643, and NGC 5861. We compare these with Hubble Space Telescope (HST) Cepheid-based relative distance moduli for the same galaxies and anchor. We find no evidence of a difference between their weighted means, 0.01 +/- 0.04 (stat) +/- 0.04 (sys) mag. We produce fourteen variants of the TRGB analysis, altering the smoothing level and color range used to measure the tips to explore their impact. For some hosts, this changes the identification of the strongest peak, but this causes little change to the sample mean difference producing a full range of 0.01 to 0.03 mag, all consistent at 1 sigma with no difference. The result matches past comparisons of I-band TRGB and Cepheids when both use HST. SNe and anchor samples observed with JWST are too small to yield a measure of H0 that is competitive with the HST sample of 42 SNe Ia and 4 anchors; however, they already provide a vital systematic crosscheck to HST measurements of the distance ladder.

==> referee_response.tex <==
Thank you for your comments, we found them to be very helpful. We have incorporated all of your suggestions into our manuscript. In addition, after we submitted our manuscript to ApJ, observations of NGC 5861 became available, and so we incorporated analysis of that galaxy into this paper. Our main result remains unchanged after including NGC 5861. Please find our responses below and in-text edits in red:

The authors present distance measurements to seven galaxies obtained using the TRGB method, calibrated with the NGC 4258 maser galaxy. Distances obtained with the TRGB method are compared with those based on Cepheids, also calibrated using the NGC 4258 data. The authors do not find any substantial difference between their weighted means.

The manuscript is written with accuracy and clarity and demonstrates high scientific standards. The results are interesting and important; however, some aspects require further clarification and discussion.


1. (l 97): reddening
- Please provide the exact values E(B-V) used for the foreground extinction correction.
- Has the color selection for the TRGB measurement been adjusted to account for the reddening correction?

Response: We have added the E(B-V) values for each galaxy in Table 2 as well as a note that the color selection has been adjusted to account for reddening on lines 100 - 101.

2. (l. 118):
"TRGB uncertainties are estimated using bootstrap resampling of the luminosity function with 100 samples."
- Is this a typo, or were the uncertainties indeed estimated with only 100 resamples? For some luminosity functions, resampling only 100 times may not accurately estimate the uncertainties associated with edge detection. Additionally, even if this number is deemed sufficient, some readers may require further justification to be convinced.

Response: We have increased the number of bootstrap samples to 5000 and updated the number on line 123.

- Please provide additional details of this estimation. Were the uncertainties estimated as the standard deviation of the distribution? Is the average or median value of the distribution close to the original measured value? Does the distribution approximate a Gaussian distribution? Those questions are especially notable for NGC5584 (Figure 3.)

Response: We have added this information starting on line 124 with an additional note about NGC 5584 starting on line 127. We find that the bootstrap distribution follows two gaussians and choose to adopt the spread in that distribution as the uncertainty to account for uncertainty in peak selection for NGC 5584.


3.
- For all analysed galaxies some basic informations are missing. What is the number of stars above/below the TRGB - preferred would be to report number of stars 1 mag. above the TRGB and either below, or as the contrast ratio (R).

Response: We've added the contrast ratio and number of stars 1 mag fainter than the TRGB in Table 2 and updated the caption to reflect this.

- What is the photometric completeness for those galaxies? Especially, for NGC 3370 seems that 50\% completeness can be quite close to the detected TRGB. Can it influence the measurement?

Response: We have added a description starting on line 146.

4.
Those results are in clear disagreement with the results presented by Freedman et al. 2024 in 'Status Report on the Chicago-Carnegie Hubble Program (CCHP): Three Independent Astrophysical Determinations of the Hubble Constant Using the James Webb Space Telescope' (https://ui.adsabs.harvard.edu/abs/2024arXiv240806153F/abstract).

While this paper is only available as a preprint, I strongly encourage the authors to reference this result and provide additional discussion on the potential sources of this discrepancy.

Response: We have added a description beginning on line 235. This description includes noting that the Freedman et al. 2024 preprint does not include the TRGB/Cepheid measurement error in NGC 4258 in their analysis; properly accounting for this places their difference at less than 1 sigma significance. In addition, the primary paper with their TRGB results, Hoyt et al., in prep, is not available precluding further comparisons.

Data Editor's Review:
One of our expert data editors has reviewed your initial manuscript submission and has the following suggestion(s) to help improve the data, software citation and/or overall content. Please treat this as you would a reviewer's comments and respond accordingly in your report to the science editor. Questions can be sent directly to the data editors at data-editors@aas.org.

a) It is great that you have minted a MAST DOI and included it in your manuscript. The next step is to mark up the DOI using the AASTeX \dataset[]{} command [1] so that the data can be properly linked in production (e.g., \dataset[DOI: 10.17909/556t-7522]{https://doi.org/10.17909/556t-7522}).

Response: We've placed the DOI in the dataset command on line 299.

[1] https://journals.aas.org/aastexguide/#datasets

b) Please additionally include the 2022 citation for Astropy: 2022ApJ...935..167A.

Response: We've added the Astropy 2022 citation on line 305.
